Lights, Camera, Matching: The Role of Image Illumination in Fair Face Recognition

Facial brightness is a key image quality factor impacting face recognition accuracy differentials across demographic groups. In this work, we aim to decrease the accuracy gap between the similarity score distributions for Caucasian and African American female mated image pairs, as measured by d' between distributions. To balance brightness across demographic groups, we conduct three experiments, interpreting brightness in the face skin region either as median pixel value or as the distribution of pixel values. Balancing based on median brightness alone yields up to a 46.8% decrease in d', while balancing based on brightness distribution yields up to a 57.6% decrease. In all three cases, the similarity scores of the individual distributions improve, with mean scores maximally improving 5.9% for Caucasian females and 3.7% for African American females.

==> exp-sections/exp1-bv/1a-and-1b.tex <==
\subsection{Analysis}

When balancing with respect to matched BVD, we find that, while all balanced subsets (e.g. N top Pairs for decreasing N) show a decrease in d', the actual d' shift is inconsistent. Thus, we conclude the following: 
\begin{itemize}
    \item Balancing across demographics with respect to ensuring that all represented pairs have the same range of BVD \textit{does} shift the distributions to higher similarity scores and decrease the d' between them.
    \item However, the actual decrease in d' is not consistent as we take ``better and better'' subsets (i.e. N top pairs with smaller N). 
\end{itemize}

When balancing with respect to matched BVC, we find that, while all balanced subsets (e.g. for a given \# Pairs) show a decrease in d', the actual d' shift is inconsistent. 

==> exp-sections/exp1-bv/1b-bvc.tex <==
\subsection{Brightness Value Combination (BVC)}\label{exp1b}

\subsubsection{BVC Balancing}
For each CF pair, we attempt to find a unique AF pair with the same BVC tuple. For only 10,454 of the CF pairs, there exists an AF pair with the same BVC. Since there is not an innate ``ordering'', we simply select 10k pairs to balance the CF and AF pairs. Tab. \ref{tab:BVC-balancing} shows the results.

==> exp-sections/exp2-bd/2a-bdm.tex <==
\section{Brightness Distribution Modality} \label{2a-bdm}

\subsection{Pre-Processing}
Each brightness distribution can be described in terms of modality: unimodal (Uni), bimodal (Bi), or multimodal (Multi). We label each image according to the modality of its brightness distribution. Our method for assigning modality is described in the Supplementary Material. 

Fig. \ref{fig:ex-uni-bi-images} shows examples from the CF / AF image sets of images with Uni distributions (``Uni'' images) and Bi distributions (``Bi'' images). On each distribution, a red x marks the peak(s) determined according to our modality-assignment method. Note that the y-axis corresponds to relative frequency and x-axis corresponds to pixel value (0-255) - these are omitted for visual clarity here. These axes are shown in the extended example in the Supplementary Material, along with a Multi example.

\begin{figure*}[!ht]
  \centering
  \includegraphics[width=.8\textwidth]{figures/exp2/ex-uni-bi-images.png}
  \caption{Example Uni / Bi / Multi images of the same CF subject.}
  \label{fig:ex-uni-bi-images}
\end{figure*}

Now that we have determined the BDM of each \textit{individual} image in each demographic, we can label each mated pair according to the BDM of its two images. This labeling allows for six possible pair Types: UniUni (UU), BiBi (BB), MultiMulti (MM), UniBi (UB), UniMulti (UM), and BiMulti (BM). 

Tab. \ref{tab:bdm-all} shows the number of pairs of each type for the two demographics (``\# of Pairs''), along with the percentage of all pairs that that type makes up for that demographic (``\% of Pairs'').

\input{tables/bdm-all}

\subsection{BDM Balancing}

In all cases where a ``Uni'' image is involved in a pair (UniUni, UniBi, UniMulti), we see either an \textit{increase} in d' or essentially no change. In all three cases, CF and AF distributions alike shift to lower match scores. Even though the distributions shift lower for both demographics, the downward shift is greater for CF, causing the increase in d'. 

With this in mind, our attempt to balance based on BDM of image pairs will consider what happens when we only take subsets of the distributions that exclude pairs with a Uni image. We will consider three groupings:
\begin{itemize}
    \item Pairs with only Bi and Multi images \\ \textit{BiBi, MultiMulti, BiMulti}
    \item Pairs that include at least one Bi image \\ \textit{BiBi, BiMulti}
    \item Pairs that include at least one Multi image \\ \textit{MultiMulti, BiMulti}
\end{itemize}

For the first and third groupings, we can balance by taking 5k, pairs each from the CF and AF distributions. For the second grouping, we are limited by the fact that Multi images in general are a small proportion of each demographic's image set, and take only 3k pairs. 

When taking our subsets, since there is no inherent ordering, we shuffle the full set of pairs each time, and average across 10 trials to get the CF / AF mean scores and d' values. The results are given in Tab. \ref{tab:bdm-balancing}.

\input{tables/bdm-bal}

==> exp-sections/exp2-bd/2b-bd-iou.tex <==
\section{Brightness Distribution Similarity}\label{2b-bdiou}
Intersection-over-union (IoU) is a measure that combines the idea of intersection with that of union. It measures the similarity between two distributions, ``rewarding'' the areas in which they are similar (overlap) and ``penalizing'' the areas in which they differ (non-overlap). So we can take the IoU of two brightness distributions (representing a pair of images) as a measure of similarity between them. 

\subsection{BD-IoU Preprocessing}

For each pair, we calculate the IoU of its two images as shown in Alg. \ref{alg:iou-only}.

%\input{exp-sections/exp2-bd/code_blocks/max_bd_iou}
\input{exp-sections/exp2-bd/code_blocks/bd-iou}

\subsubsection{BD-IoU Balancing}




==> exp-sections/exp2-bd/code_blocks/bvd-bvc.tex <==
\RestyleAlgo{ruled}

%% This is needed if you want to add comments in
%% your algorithm with \Comment
\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}[hbt!]
\caption{BVD \& BVC of Image Pair}\label{alg:bvd}
\vspace{0.25em}
\KwData{$BV_{1}, BV_{2}$}
\KwResult{$BVD_{1,2}, BVC_{1,2}$}
\vspace{0.5em}
$BVD_{1,2} \gets \lvert BV_1 - BV_2 \rvert$\;
\vspace{0.5em}
$LBV \gets min(BV_1,BV_2)$\; 
$HBV \gets max(BV_1,BV_2)$\;
$BVC_{1,2} \gets (LBV,HBV)$
\vspace{0.25em}
\end{algorithm}

==> figures/exp1/bvd-bvc-ex.tex <==
\begin{figure}[!ht]
    \centering
    \includegraphics[width=.75\columnwidth]{figures/exp1/bvd-bvc-example.png}
    \caption{Ex. image pair with BVD and BVC values.}
    \label{fig:bvd-bvc-ex}
\end{figure}

==> figures/exp2/AF-CF-bdmPAIRS-bdiou.tex <==
\begin{figure*}[!ht]
  \centering
  \includegraphics[width=\textwidth]{figures/exp2/af-cf-bdmPAIRTYPE-bdiou.png}
  \caption{For CF and AF, the percentage of pairs from each BDM pair type (UniUni, BiBi, MultiMulti, UniBi, UniMulti, BiMulti) in all images vs. in the BDIoU-balanced N Top Pairs Groups.}
  \label{fig:cf-af-bdmPAIRS-bdiou}
\end{figure*}

==> figures/exp2/bdm-histogram-ex.tex <==
\begin{figure*}[!ht]
  \centering
  \includegraphics[width=.75\textwidth]{figures/exp2/bdm-histogram-example.png}
  \caption{Generation of a binned histogram (for determining BDM) and smoothed histogram (for determining BD-IOU).}
  \label{fig:bdm-hist-ex}
\end{figure*}

==> figures/exp2/ex-only-af-bdm-bdiou.tex <==
\begin{figure*}[!ht]
  \centering
  \includegraphics[width=\textwidth]{figures/exp2/ex-afonly-bdiou-bdm.png}
  \caption{For AF, the percentage of images from each BDM type (Uni, Bi, Multi) in all images vs. in the BDIoU-balanced N Top Pairs Groups.}
  \label{fig:ex-af-bdiou-bdm-perc}
\end{figure*}

==> sections/dataset.tex <==
\section{Dataset and Preprocessing}\label{dataset}



==> tables/FINAL-bdiou-bdm.tex <==
\begin{table}[]
\caption{For the N Top Pairs, shift in score mean, shift in d', and mean BD-IoU.}
\label{tab:bdiou-bdm}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|ccccc|}
\hline
\multicolumn{5}{|c|}{\cellcolor[HTML]{CBCEFB}\textbf{Balancing Factor: BD-IoU + BDM}} \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}N Top\\ Pairs\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Dem.}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Score $\bar{x}$\\ Shift\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}d'\\ Shift\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}BD-IoU\\ $\bar{x}$\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{3k}} & \multicolumn{1}{c|}{CF} & \multicolumn{1}{c|}{3.8\%} & \multicolumn{1}{c|}{\multirow{2}{*}{-31.5\%}} & \multirow{2}{*}{0.87} \\ \cline{2-3}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{AF} & \multicolumn{1}{c|}{1.8\%} & \multicolumn{1}{c|}{} &  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{2k}} & \multicolumn{1}{c|}{CF} & \multicolumn{1}{c|}{4.5\%} & \multicolumn{1}{c|}{\multirow{2}{*}{-30.6\%}} & \multirow{2}{*}{0.88} \\ \cline{2-3}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{AF} & \multicolumn{1}{c|}{2.5\%} & \multicolumn{1}{c|}{} &  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{1k}} & \multicolumn{1}{c|}{CF} & \multicolumn{1}{c|}{5.9\%} & \multicolumn{1}{c|}{\multirow{2}{*}{-41.0\%}} & \multirow{2}{*}{0.90} \\ \cline{2-3}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{AF} & \multicolumn{1}{c|}{3.2\%} & \multicolumn{1}{c|}{} &  \\ \hline
\end{tabular}%
}
\end{table}

==> tables/bdiou.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[!ht]
\caption{For the N Top Pairs, shift in score mean, shift in d', and mean BD-IoU.}
\label{tab:bdiou}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|ccccc|}
\hline
\multicolumn{5}{|c|}{\cellcolor[HTML]{CBCEFB}\textbf{Balancing Factor: BD-IoU}} \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}N Top\\ Pairs\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Dem.}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Score $\bar{x}$\\ Shift\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}d'\\ Shift\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}BD-IoU\\ $\bar{x}$\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{10k}} & \multicolumn{1}{c|}{CF} & \multicolumn{1}{c|}{1.2\%} & \multicolumn{1}{c|}{\multirow{2}{*}{-16.5\%}} & \multirow{2}{*}{0.85} \\ \cline{2-3}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{AF} & \multicolumn{1}{c|}{0.2\%} & \multicolumn{1}{c|}{} &  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{5k}} & \multicolumn{1}{c|}{CF} & \multicolumn{1}{c|}{2.5\%} & \multicolumn{1}{c|}{\multirow{2}{*}{-25.1\%}} & \multirow{2}{*}{0.88} \\ \cline{2-3}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{AF} & \multicolumn{1}{c|}{1.0\%} & \multicolumn{1}{c|}{} &  \\ \hline
\multicolumn{1}{|c|}{\multirow{2}{*}{1k}} & \multicolumn{1}{c|}{CF} & \multicolumn{1}{c|}{5.3\%} & \multicolumn{1}{c|}{\multirow{2}{*}{-38.7\%}} & \multirow{2}{*}{0.90} \\ \cline{2-3}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{AF} & \multicolumn{1}{c|}{2.8\%} & \multicolumn{1}{c|}{} &  \\ \hline
\end{tabular}%
}
\end{table}

==> tables/bvc-bal.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[!ht]
\caption{Same-size subsets of CF and AF.}
\label{tab:BVC-balancing}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|ccccc|}
\hline
\multicolumn{5}{|c|}{\cellcolor[HTML]{EFEFEF}\textbf{Bal. Factor: BVC}} \\ \hline
\multicolumn{1}{|c|}{\textbf{\begin{tabular}[c]{@{}c@{}}N Sel.\\ Pairs\end{tabular}}} & \multicolumn{1}{c|}{\textbf{Dem.}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Score $\bar{x}$\\ Shift\end{tabular}}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}d'\\ Shift\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}BVD\\ $\bar{x}$\end{tabular}} \\ \hline
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{CF} & \multicolumn{1}{c|}{0.86\%} & \multicolumn{1}{c|}{} &  \\ \cline{2-3}
\multicolumn{1}{|c|}{\multirow{-2}{*}{10k}} & \multicolumn{1}{c|}{AF} & \multicolumn{1}{c|}{0.64\%} & \multicolumn{1}{c|}{\multirow{-2}{*}{-1.80\%}} & \multirow{-2}{*}{26.0} \\ \hline
\end{tabular}%
}
\end{table}
